Persian Abstract Meaning Representation: Annotation Guidelines and Gold Standard Dataset

This paper introduces the Persian Abstract Meaning Representation (AMR) guidelines, a detailed guide for annotating Persian sentences with AMR, focusing on the necessary adaptations to fit Persian's unique syntactic structures. We discuss the development process of a Persian AMR gold standard dataset consisting of 1,562 sentences created following the guidelines. By examining the language specifications and nuances that distinguish AMR annotations of a low-resource language like Persian, we shed light on the challenges and limitations of developing a universal meaning representation framework. The guidelines and the dataset introduced in this study highlight such challenges, aiming to advance the field.

==> 01titlepage.tex <==
\title{Persian Abstract Meaning Representation
%\thanks{}
}
% Grants or other notes about the article that should go on the front
% page should be placed within the \thanks{} command in the title
% (and the %-sign in front of \thanks{} should be deleted)
%
% General acknowledgments should be placed at the end of the article.

%\subtitle{Do you have a subtitle?\\ If so, write it here}

%\titlerunning{Short form of title}        % if too long for running head

\author{Reza Takhshid         \and
        Razieh Shojaei \and
        Zahra Azin \and
        Mohammad Bahrani
}

%\authorrunning{Short form of author list} % if too long for running head

\institute
{
Reza Takhshid: M.Sc. Graduate in Computational\at Sharif University of Technology   \\  \email{reza.takhshid95@student.sharif.edu} 
\and
Razieh Shojaei: Ph.D. Graduate in Linguistics, \at University of Tehran\\ \email{rshojae@alumni.ut.ac.ir} 
 \and
 Zahra Azin: M.Sc. Graduate in Computational Linguistics,\at Sharif University of Technology
\\ \email{z\_azin@alum.sharif.ir}
\and
Mohammad Bahrani: Assistant professor, \at Faculty of Mathematical Sciences \& Computer, Allameh Tabataba’i University
\\
\email{bahrani@atu.ac.ir}
}
\date{Received: date / Accepted: date}
% The correct dates will be entered by the editor


